NovaCOMET: Open Commonsense Foundation Models with Symbolic Knowledge Distillation

We present NovaCOMET, an open commonsense knowledge model, that combines the best aspects of knowledge and general task models. Compared to previous knowledge models, NovaCOMET allows open-format relations enabling direct application to reasoning tasks; compared to general task models like Flan-T5, it explicitly centers knowledge, enabling superior performance for commonsense reasoning. NovaCOMET leverages the knowledge of opaque proprietary models to create an open knowledge pipeline. First, knowledge is symbolically distilled into NovATOMIC, a publicly-released discrete knowledge graph which can be audited, critiqued, and filtered. Next, we train NovaCOMET on NovATOMIC by fine-tuning an open-source pretrained model. NovaCOMET uses an open-format training objective, replacing the fixed relation sets of past knowledge models, enabling arbitrary structures within the data to serve as inputs or outputs. The resulting generation model, optionally augmented with human annotation, matches or exceeds comparable open task models like Flan-T5 on a range of commonsense generation tasks. NovaCOMET serves as a counterexample to the contemporary focus on instruction tuning only, demonstrating a distinct advantage to explicitly modeling commonsense knowledge as well.

==> sections/methods.tex <==
\section{Methods}
\label{sec:methods}

==> sections/related_OLD.tex <==
\section{[PREVIOUS RELATED WORK]}

\paragraph{General Language Model Tuning:} \peter{Other methods for turning LMs into cross-task models}

flan: \url{https://arxiv.org/pdf/2210.11416.pdf}


%Scale flan: \url{https://openreview.net/pdf?id=gEZrGCozdqR]

unicorn

macaw

unified qa

cross-fit


\paragraph{Symbolic Knowledge Distillation and Data Generation:} 
While manual dataset creation is expensive and complex, previous works have looked into automatic data generation. Earlier work mainly focus on extractive approaches, e.g. syntactic parsing \cite{Zhang2020TransOMCSFL} or pattern matching \cite{causalbank} from unstructured text \cite{Lehmann2015DBpediaA, buck2014n}. %These a0scale, but are noisyRecent work 

\peter{Our previous work, Melanie's paper etc. Focus on things that distill some specific aspect, but also some famous data generation like the Schutze paper.}

melanie's summarization work

wanli

soda

\liwei{left some references}
\begin{itemize}
    \item Commonsense: symbolic knowledge distillation \url{https://arxiv.org/abs/2110.07178}, using critic model to filter low quality data
    \item Summarization: referee \url{https://arxiv.org/abs/2210.13800}, iterative data distillation
    \item Summarization: Impossible Distillation \url{https://arxiv.org/abs/2305.16635}, distill from small models
    \item Generics: i2d2 \url{https://arxiv.org/abs/2212.09246}, iterative model distillation with controllable decoding
    \item NLI: wanli \url{https://arxiv.org/abs/2201.05955}, human-ai collaborative dataset creation
    \item Dialogue: SODA \url{https://arxiv.org/abs/2212.10465}, staged distillation from commonsense knowledge tuples => narratives expanded from commonsense knowledge => narrative grounded dialogues
    \item Dialogue: Baze \url{https://arxiv.org/abs/2304.01196}
    \item Dialogue: Koala \url{https://bair.berkeley.edu/blog/2023/04/03/koala/}
    \item Dialogue: Vicuna \url{https://lmsys.org/blog/2023-03-30-vicuna/}
    \item Chain-of-Thought: Symbolic Chain-of-Thought Distillation \url{https://arxiv.org/abs/2110.07178} \liwei{i'm not super sure about this one so it'll be great to take a look.}
\end{itemize}





\paragraph{Commonsense Knowledge Modeling:} \peter{Stuff like COMET, ATOMIC, causalbank. Perhaps also include the Graham Neubig papers on treating models as KBs, although maybe this fits in data generation }
\peter{Also, include just a couple of papers that go beyond text-only. Like visualcomet}

\peter{Not sure if this goes here, but another knowledge modeling (COMET) paper that evals on tellmewhy: https://openreview.net/pdf?id=H4xz8zteub9}

==> tables/QA_results_v0.tex <==
\begin{table*}[t!]
    \centering\footnotesize
     \scalebox{.98}{
    \begin{tabular}{l|ccccccccccc}
\toprule
               system &  HW &  aNLI &  CODAH &  WG &  CSQA &  csqa2 &  SIQA &  CosmosQA &  RS &  PIQA \\
\midrule
     t5-xxl &       45.7 &  61.3 &   46.8 &        53.4 &  40.2 &   51.3 &  41.4 &      29.6 &         17.9 &  75.5 \\
flan-t5-xxl &       52.3 &  62.5 &   58.4 &        83.8 &  69.5 &   56.4 &  55.9 &      23.8 &         34.1 &  77.8 \\
         t0 &       45.9 &  59.5 &   42.2 &        59.6 &  58.9 &   51.2 &  53.9 &      22.9 &         30.9 &  73.4 \\
  llama-13b &       55.2 &  62.9 &   42.5 &        50.7 &  41.2 &   49.1 &  42.0 &      27.8 &         27.8 &  73.9 \\
      macaw &       41.6 &  61.6 &   45.1 &        50.3 &  26.2 &   51.8 &  40.3 &      32.5 &         15.4 &  74.1 \\
   llama-7b &       51.9 &  62.7 &   40.6 &        50.5 &  43.8 &   49.2 &  42.7 &      26.3 &         25.2 &  72.0 \\
   flan-ul2 &       57.3 &  64.1 &   59.0 &        82.6 &  69.1 &   56.1 &  58.9 &      25.2 &         35.0 &  78.8 \\
   \midrule
          100k\_critic &       64.2 &  73.6 &   83.2 &        78.1 &  73.1 &   53.3 &  70.1 &      81.0 &         54.6 &  80.2 \\
\bottomrule
    \end{tabular}}
    \caption{ Comparison using \emph{absolute scores} from different models. 
    % GPT-3 and GPT-3 Instruct refer to the \texttt{davinci} and \texttt{text-davinci-002} engines on the OpenAI API, respectively.
    }
    \label{tab:modularity_combined}
\end{table*}

==> tables/generation_auto_old.tex <==
\begin{table*}[t!]
    \centering\footnotesize
     \scalebox{.98}{
    \begin{tabular}{lrrrrr}
\toprule
                  system &  anlg &  csqg &  reflect &  atomic &   tmw \\
\midrule
       greedy\_alpaca-13b & 0.749 & 0.739 &    0.724 &   0.697 & 0.780 \\
           greedy\_t5-xxl & 0.742 & 0.730 &    0.657 &   0.681 & 0.718 \\
        greedy\_alpaca-7b & 0.694 & 0.738 &    0.739 &   0.701 & 0.789 \\
      greedy\_flan-t5-xxl & 0.789 & 0.798 &    0.757 &   0.726 & 0.801 \\
               greedy\_t0 & 0.742 & 0.784 &    0.772 &   0.715 & 0.767 \\
        greedy\_llama-13b & 0.720 & 0.658 &    0.698 &   0.671 & 0.734 \\
         greedy\_llama-7b & 0.705 & 0.648 &    0.686 &   0.670 & 0.737 \\
greedy\_nova\_comet\_gen\_r0 & 0.756 & 0.789 &    0.753 &   0.730 & 0.810 \\
         greedy\_flan-ul2 & 0.789 & 0.793 &    0.696 &   0.715 & 0.684 \\
greedy\_nova\_comet\_gen\_r1 & 0.747 & 0.786 &    0.746 &   0.726 & 0.807 \\
\midrule
           greedy\_may15\_none\_human20k\_round0\_cp30k & 0.744 & 0.774 &    0.757 &   0.751 & 0.790 \\
          greedy\_may11\_feb28\_gen\_newgen\_mix\_cp\_50k & 0.748 & 0.779 &    0.758 &   0.751 & 0.791 \\
         greedy\_may15\_nonone\_human20k\_round0\_cp70k & 0.734 & 0.760 &    0.754 &   0.751 & 0.789 \\
         greedy\_march1\_feb28\_gen\_newgen\_mix\_cp120k & 0.774 & 0.782 &    0.761 &   0.748 & 0.800 \\
            greedy\_april2\_april\_2\_gpt3turbo\_cp200k & 0.789 & 0.789 &    0.771 &   0.725 & 0.811 \\
greedy\_may16\_none\_human20k\_round0\_cp90k\_INCOMPLETE & 0.752 & 0.772 &    0.759 &   0.749 & 0.798 \\
greedy\_may18\_none\_human20k\_round0\_cp40k\_INCOMPLETE & 0.752 & 0.774 &    0.757 &   0.743 & 0.797 \\
greedy\_may19\_turbo\_lr0\_0001\_bs256\_human20k\_roun... & 0.787 & 0.789 &    0.772 &   0.725 & 0.810 \\
     greedy\_april2\_april\_2\_gpt3turbo\_cp80k\_PARTIAL & 0.792 & 0.791 &    0.771 &   0.724 & 0.810 \\
\bottomrule
    \end{tabular}}
    \caption{ Comparison using \emph{absolute scores} from different models. 
    % GPT-3 and GPT-3 Instruct refer to the \texttt{davinci} and \texttt{text-davinci-002} engines on the OpenAI API, respectively.
    }
    \label{tab:modularity_combined}
\end{table*}

==> tables/question_example_old.tex <==
\begin{table}[t!]
\small
\centering % @{\hspace{0.6\tabcolsep}}
    \begin{tabular}{l@{\hspace{0.6\tabcolsep}}}
    % |l@{\hspace{0.6\tabcolsep}}}
        \toprule 

            % \multirow{3}{*}{\makecell[tl]{\textbf{Dataset}}} &       &  \multicolumn{4}{c|}{\textbf{Premise/Event}} & \multicolumn{4}{c|}{\textbf{Question/Relation}} & \multicolumn{4}{c}{\textbf{Hypothesis/Tail}} \\

            % \multirow{2}{*}{\makecell[tl]{Type}} & \multirow{2}{*}{\makecell[tl]{Dataset \\ \textsc{Atomic}}} &  \multicolumn{2}{c|}{\textbf{Entries}} & \multicolumn{2}{c}{\textbf{3-grams}}  \\

            %  &  & \# & \% & \# & \% \\

            \textbf{Most Frequent Questions} \\
            \midrule
        
            what time of day is it? \\
            what is the weather like? \\
            who is personx? \\
            who is persony? \\
            what time is it? \\ 
            what is the occasion? \\ 
            what is the relationship between personx and persony? \\
            what is the prerequisite for this situation? \\ 
            what is the counterfactual of the situation? \\ 
            what is personx doing? \\
            what is a prerequisite for this situation? \\
            what is the time of day? \\

        \bottomrule
    \end{tabular}
    \caption{Most frequent questions in the dataset.}
\label{tab:question-example}
\end{table}


